Volumes in Hyperbolic Space

This paper focuses on the investigation of volumes of large Coxeter hyperbolic polyhedron. First, the paper investigates the smallest possible volume for a large Coxeter hyperbolic polyhedron and then looks at the volume of pyramids with one vertex at infinity.

==> cyrillic.tex <==
\def\fileversion{1.0}
\def\filedate{2000/12/5}
\def\docdate{2000/12/5}
\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{cyrillic}[\filedate\space\fileversion\space LaTeX2e package for cyrillic fonts]

% see Helmut Kopka LaTeX Band 2 pp. 105-112

\chardef\tempcat=\the\catcode`\@
\catcode`\@=11

\def\@gobble#1{}
\def\@testgrave{\`}
\def\@stressit{\futurelet\chartest\@stresschar }

\def\@stresschar#1{%
  \ifx #1y\def\result{\futurelet\chartest\@yligature}%
  \else \ifx #1Y\def\result{\futurelet\chartest\@Yligature}%
  \else \ifx\chartest\@testgrave \def\result{\accent"26 }%
  \else \def\result{\accent"26 #1}%
  \fi \fi \fi
  \result }

\def\@yligature{%
  \ifx a\chartest \def\result{\accent"26 \char"1F \@gobble}%
  \else \ifx u\chartest \def\result{\accent"26 \char"18 \@gobble}%
  \else \def\result{\accent"26 y}%
  \fi \fi
  \result }

\def\@Yligature{%
  \ifx a\chartest \def\result{\accent"26 \char"17 \@gobble}%
  \else \ifx A\chartest \def\result{\accent"26 \char"17 \@gobble}%
  \else \ifx u\chartest \def\result{\accent"26 \char"10 \@gobble}%
  \else \ifx U\chartest \def\result{\accent"26 \char"10 \@gobble}%
  \else \def\result{\accent"26 Y}%
  \fi \fi \fi \fi
  \result }

\def\!{\ifmmode \mskip-\thinmuskip \fi}

\def\cyracc{%
  \chardef\i="10%
  \def\cydot{{\kern0pt}}%
  \def\cprime{\char"7E }\def\Cprime{\char"5E }%
  \def\cdprime{\char"7F }\def\Cdprime{\char"5F }%
  \def\dbar{dj}\def\Dbar{Dj}%
  \def\dz{\char"1E }\def\Dz{\char"16 }%
  \def\dzh{\char"0A }\def\Dzh{\char"02 }%
  \def\'##1{\if c##1\char"0F %
    \else \if C##1\char"07 %
    \else \accent"26 ##1\fi \fi }%
  \def\`##1{\if e##1\char"0B %
    \else \if E##1\char"03 %
    \else \errmessage{accent \string\` not defined in cyrillic}%
        ##1\fi \fi }%
  \def\=##1{\if e##1\char"0D %
    \else \if E##1\char"05 %
    \else \if \i##1\char"0C %
    \else \if I##1\char"04 %
    \else \errmessage{accent \string\= not defined in cyrillic}%
        ##1\fi \fi \fi \fi }%
  \def\u##1{\if \i##1\accent"24 i%
    \else \accent"24 ##1\fi }%
  \def\"##1{\if \i##1\accent"20 \char"3D %
    \else \if I##1\accent"20 \char"04 %
    \else \accent"20 ##1\fi \fi }%
  \def\!{\ifmmode \def\result{\mskip-\thinmuskip}%
    \else \def\result{\@stressit}\fi \result}}

\def\keep@cyracc{\let\cyr=\relax \let\i=\relax
        \let\ubar=\relax \let\cydot=\relax
        \let\cprime=\relax \let\Cprime=\relax
        \let\cdprime=\relax \let\Cdprime=\relax
        \let\dbar=\relax \let\Dbar=\relax
        \let\dz=\relax \let\Dz=\relax
        \let\dzh=\relax \let\Dzh=\relax
        \let\'=\relax \let\`=\relax \let\==\relax
        \let\u=\relax \let\"=\relax \let\!=\relax }

\DeclareFontEncoding{OT2}{\cyracc}{}

\DeclareOption{cyronly}{%
  \renewcommand{\encodingdefault}{OT1}
  \newcommand{\lrmfamily}{\fontencoding{OT1}\fontfamily{\rmdefault}\selectfont}
  \newcommand{\lsffamily}{\fontencoding{OT1}\fontfamily{\sfdefault}\selectfont}
  \newcommand{\lbfseries}{\fontencoding{OT1}\fontseries{\bfdefault}\selectfont}
  \newcommand{\lmdseries}{\fontencoding{OT1}\fontseries{\mddefault}\selectfont}
  \newcommand{\litshape}{\fontencoding{OT1}\fontshape{\itdefault}\selectfont}
  \newcommand{\lslshape}{\fontencoding{OT1}\fontshape{\sldefault}\selectfont}
  \newcommand{\lscshape}{\fontencoding{OT1}\fontshape{\scdefault}\selectfont}
  \newcommand{\lupshape}{\fontencoding{OT1}\fontshape{\updefault}\selectfont}
  \newcommand{\lem}{\fontencoding{OT1}\em}
  \DeclareTextFontCommand{\textlrm}{\lrmfamily}
  \DeclareTextFontCommand{\textlsf}{\lsffamily}
  \DeclareTextFontCommand{\textlbf}{\lbfseries}
  \DeclareTextFontCommand{\textlmd}{\lmdseries}
  \DeclareTextFontCommand{\textlit}{\litshape}
  \DeclareTextFontCommand{\textlsl}{\lslshape}
  \DeclareTextFontCommand{\textlsc}{\lscshape}
  \DeclareTextFontCommand{\textlup}{\lupshape}
  \DeclareTextFontCommand{\lemph}{\lem}
}

\DeclareOption{cyrpart}{%
  \newcommand{\cyrrmfamily}{\fontencoding{OT2}\fontfamily{cmr}\selectfont}
  \newcommand{\cyrsffamily}{\fontencoding{OT2}\fontfamily{cmss}\selectfont}
  \newcommand{\cyrbfseries}{\fontencoding{OT2}\fontseries{b}\selectfont}
  \newcommand{\cyrmdseries}{\fontencoding{OT2}\fontseries{m}\selectfont}
  \newcommand{\cyritshape}{\fontencoding{OT2}\fontshape{it}\selectfont}
  \newcommand{\cyrslshape}{\fontencoding{OT2}\fontshape{sl}\selectfont}
  \newcommand{\cyrscshape}{\fontencoding{OT2}\fontshape{sc}\selectfont}
  \newcommand{\cyrupshape}{\fontencoding{OT2}\fontshape{up}\selectfont}
  \newcommand{\cyrem}{\fontencoding{OT2}\em}
  \DeclareTextFontCommand{\textcyrrm}{\cyrrmfamily}
  \DeclareTextFontCommand{\textcyrsf}{\cyrsffamily}
  \DeclareTextFontCommand{\textcyrbf}{\cyrbfseries}
  \DeclareTextFontCommand{\textcyrmd}{\cyrmdseries}
  \DeclareTextFontCommand{\textcyrit}{\cyritshape}
  \DeclareTextFontCommand{\textcyrsl}{\cyrslshape}
  \DeclareTextFontCommand{\textcyrsc}{\cyrscshape}
  \DeclareTextFontCommand{\textcyrup}{\cyrupshape}
  \DeclareTextFontCommand{\emcyr}{\cyem}
}

\ExecuteOptions{cyrpart}
\ProcessOptions

\catcode`\@=\tempcat
\endinput


